Design and FPGA Implementation of WOMBAT: A Deep Neural Network Level-1 Trigger System for Jet Substructure Identification and Boosted $H\rightarrow b\bar{b}$ Tagging at the CMS Experiment

This thesis investigates the physics performance, trigger efficiency, and Field Programmable Gate Array (FPGA) implementation of machine learning (ML)-based algorithms for Lorentz-boosted $H\rightarrow b\bar{b}$ tagging within the CMS Level-1 Trigger (L1T) under Phase-1 conditions. The proposed algorithm, WOMBAT (Wide Object ML Boosted Algorithm Trigger), comprises a high-performance Master Model (W-MM) and a quantized, FPGA-synthesizable Apprentice Model (W-AM), benchmarked against the standard Single Jet 180 and the custom rule-based JEDI (Jet Event Deterministic Identifier) triggers. All algorithms process calorimeter trigger primitive data to localize boosted $H\rightarrow b\bar{b}$ jets. Outputs are post-processed minimally to yield real-valued $(\eta, \phi)$ jet coordinates at trigger tower granularity. Trigger rates are evaluated using 2023 CMS ZeroBias data (0.64 fb$^{-1}$), with efficiency assessed via a Monte Carlo sample of $H\rightarrow b\bar{b}$ offline reconstructed AK8 jets. W-MM achieves a 1 kHz rate at an offline jet $p_T$ threshold of 146.8 GeV, 40.6 GeV lower than Single Jet 180, while maintaining comparable signal efficiency. W-AM reduces the threshold further to 140.4 GeV, with reduced efficiency due to fixed-output constraints and limited multi-jet handling. FPGA implementation targeting the Xilinx Virtex-7 XC7VX690T confirms that W-AM meets resource constraints with a pre-place-and-route latency of 22 clock cycles (137.5 ns). In contrast, JEDI requires excessive resource usage and a 56-cycle latency, surpassing the 14-cycle L1T budget. Originally developed for Run-3 CMS L1T, WOMBAT serves as a proof-of-concept for Phase-2 triggers, where hardware advances will enable online deployment of more sophisticated ML-based L1T systems.

==> sections/foreword.tex <==
\setcounter{section}{-1}
\section{\colorbox{white}{\parbox[c][0.08cm][c]{0.08cm}{}}Preface}


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{sections/images/WOMBATlogoMini.png}
    \caption{Project WOMBAT Logo designed by M. Bileska}
    \label{fig:enter-label}
\end{figure}


What will go in this section after the entire thesis is complete:
\begin{itemize}
    \item An introduction of what the main point of the thesis is. Clearly spelled in a sentence or two, as a summary of the abstract in a sense.
    \item A note on how this text is organized. WOMBAT doesn't come into play until way later, but it is important for the reader to have a large overview of the detector and physics behind it. This will need to be emphasized. It is basically a \textit{please stick with me, all of the initial discussion has a purpose and this is what that purpose is.}
    \item Some other notes that may be of relevance before the reading starts.
\end{itemize}

==> sections/notes.tex <==
\section{ML Algo}

{\small Note: I will start slowly compiling all that I have done in terms of testing and parameter choosing on the (as of now) finalized V1 model. I will also re-do the tests since initially they were meant for visualization and I did not save the numerical data, only visual.}




\subsection{WOMBAT.V1 Specs}


\begin{itemize}
    \item Data \textbf{must} be preprocessed to apply the $-30.0\;GeV$ threshold. This is not difficult to implement on the model, but $hls4ml$ has a vendetta against custom layers or even the function $Subtract$ for tf tensors. I tried essentially all that I could think of, and yes, there is a way to integrate a custom layer in hls, but it requires additions to the nnet directory, which I will skip for now. At this point, I just want to implement the V1 model in fpgas.
\end{itemize}


\textbf{Model Configuration:}

\begin{itemize}
    \item \textbf{Input Layer}
    \begin{itemize}
        \item \textbf{Type}: Input
        \item \textbf{Shape}: (18, 14, 1)
        \item \textbf{Name}: inputs
    \end{itemize}
    
    \item \textbf{Layer 1: Convolutional Layer}
    \begin{itemize}
        \item \textbf{Type}: QConv2D
        \item \textbf{Filters}: 32
        \item \textbf{Kernel Size}: (3, 3)
        \item \textbf{Padding}: same
        \item \textbf{Kernel Quantization}: quantized\_bits(8, 1, 1, alpha=1)
        \item \textbf{Bias Quantization}: quantized\_bits(8, 1, 1, alpha=1)
        \item \textbf{Name}: conv\_1
    \end{itemize}
    
    \item \textbf{Layer 2: Batch Normalization}
    \begin{itemize}
        \item \textbf{Type}: BatchNormalization
        \item \textbf{Name}: norm\_1
    \end{itemize}
    
    \item \textbf{Layer 3: Activation Layer}
    \begin{itemize}
        \item \textbf{Type}: QActivation
        \item \textbf{Activation}: quantized\_relu(8)
        \item \textbf{Name}: relu\_1
    \end{itemize}
    
    \item \textbf{Layer 4: Pooling Layer}
    \begin{itemize}
        \item \textbf{Type}: AveragePooling2D
        \item \textbf{Pool Size}: (2, 2)
        \item \textbf{Name}: pool\_1
    \end{itemize}
    
    \item \textbf{Layer 5: Convolutional Layer}
    \begin{itemize}
        \item \textbf{Type}: QConv2D
        \item \textbf{Filters}: 64
        \item \textbf{Kernel Size}: (3, 3)
        \item \textbf{Padding}: same
        \item \textbf{Kernel Quantization}: quantized\_bits(8, 1, 1, alpha=1)
        \item \textbf{Bias Quantization}: quantized\_bits(8, 1, 1, alpha=1)
        \item \textbf{Name}: conv\_2
    \end{itemize}
    
    \item \textbf{Layer 6: Batch Normalization}
    \begin{itemize}
        \item \textbf{Type}: BatchNormalization
        \item \textbf{Name}: norm\_2
    \end{itemize}
    
    \item \textbf{Layer 7: Activation Layer}
    \begin{itemize}
        \item \textbf{Type}: QActivation
        \item \textbf{Activation}: quantized\_relu(8)
        \item \textbf{Name}: relu\_2
    \end{itemize}
    
    \item \textbf{Layer 8: Pooling Layer}
    \begin{itemize}
        \item \textbf{Type}: AveragePooling2D
        \item \textbf{Pool Size}: (2, 2)
        \item \textbf{Name}: pool\_2
    \end{itemize}
    
    \item \textbf{Layer 9: Flatten Layer}
    \begin{itemize}
        \item \textbf{Type}: Flatten
        \item \textbf{Name}: flatten\_1
    \end{itemize}
    
    \item \textbf{Layer 10: Dense Layer}
    \begin{itemize}
        \item \textbf{Type}: QDense
        \item \textbf{Units}: 128
        \item \textbf{Kernel Quantization}: quantized\_bits(8, 1, 1, alpha=1)
        \item \textbf{Bias Quantization}: quantized\_bits(8, 1, 1, alpha=1)
        \item \textbf{Name}: dense\_1
    \end{itemize}
    
    \item \textbf{Layer 11: Activation Layer}
    \begin{itemize}
        \item \textbf{Type}: QActivation
        \item \textbf{Activation}: quantized\_relu(8)
        \item \textbf{Name}: relu\_3
    \end{itemize}
    
    \item \textbf{Layer 12: Dropout Layer}
    \begin{itemize}
        \item \textbf{Type}: Dropout
        \item \textbf{Rate}: 0.5
    \end{itemize}
    
    \item \textbf{Layer 13: Output Layer}
    \begin{itemize}
        \item \textbf{Type}: QDense
        \item \textbf{Units}: 4
        \item \textbf{Kernel Quantization}: quantized\_bits(8, 1, 1, alpha=1)
        \item \textbf{Bias Quantization}: quantized\_bits(8, 1, 1, alpha=1)
        \item \textbf{Name}: dense\_out
    \end{itemize}
\end{itemize}

Early Stopping is implemented with a tolerance of $10$.

{\small Note: no regularizer added yet, $R^2$ score decreased with a regularizer but it can be a future consideration.}


\textbf{Current args:}

\begin{itemize}
    \item \textbf{Argument 1: H5 Filename}
    \begin{itemize}
        \item \textbf{Type}: str
        \item \textbf{Description}: Path to the H5 file
        \item \textbf{Variable Name}: h5\_filename
    \end{itemize}

    \item \textbf{Argument 2: Number of Epochs}
    \begin{itemize}
        \item \textbf{Type}: int
        \item \textbf{Description}: Number of epochs
        \item \textbf{Variable Name}: epochs
    \end{itemize}

    \item \textbf{Argument 3: Batch Size}
    \begin{itemize}
        \item \textbf{Type}: int
        \item \textbf{Description}: Batch size
        \item \textbf{Variable Name}: batch\_size
    \end{itemize}
\end{itemize}









\section{FPGA Implementation}
